Simulation-Based Digital Twin Development for Blockchain Enabled End-to-End Industrial Hemp Supply Chain Risk Management

With the passage of the 2018 U.S. Farm Bill, Industrial Hemp production is moved from limited pilot programs to a regulated agriculture production system. However, Industrial Hemp Supply Chain (IHSC) faces critical challenges, including: high complexity and variability, very limited production knowledge, lack of data and information tracking. In this paper, we propose blockchain-enabled IHSC and develop a preliminary simulation-based digital twin for this distributed cyber-physical system (CPS) to support the process learning and risk management. Basically, we develop a two-layer blockchain with proof of authority smart contract, which can track the data and key information, improve the supply chain transparency, and leverage local authorities and state regulators to ensure the quality control verification. Then, we introduce a stochastic simulation-based digital twin for IHSC risk management, which can characterize the process spatial-temporal causal interdependencies and dynamic evolution to guide risk control and decision making. Our empirical study demonstrates the promising performance of proposed platform.

==> latexmacro.tex <==

%% LaTeX2e file `latexmacro.tex'
%% generated by the `filecontents' environment
%% from source `Gkmn51' on 2001/03/06.
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  This macro contains definitions of new \LaTeX commands  %%
%%  that are frequently used by Barry L. Nelson.  This is   %%
%%  a new release of the 'latexmacro.tex' file that I have  %%
%%  distributed for some time.  This release                %%
%%  is designed to be compatible with previous releases,    %%
%%  except for eliminating the \smallheads command.         %%
%%                                                          %%
%%  This releases fixes a few bugs (please report any you   %%
%%  find to nelsonb@random.eng.ohio-state.edu), includes    %%
%%  more documentation, and completes the definitions of    %%
%%  bold-face mathematics characters.                       %%
%%                                                          %%
%%  release 2.01   1/2/92                                   %%
%%  unreleased update 6/9/92  6/22/92 1/19/93 2/3/93        %%
%%                    6/2/93  8/15/93 11/11/93 11/23/93     %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% USING THE MACRO:
%% If you name this file latexmacro.tex, then use the following
%% statement just after the \documentstyle{} command:
%%
%%    \input [path] latexmacro
%%
%% LINE SPACING:
%% Define single, one and a half, and double space commands; these
%% may be used anywhere after \begin{document}
%%
\def\double{\par\baselineskip=24pt}
\def\single{\par\baselineskip=12pt}
\def\oneandahalf{\par\baselineskip=18pt}
%%
%% TEXT DIMENSIONS
%% Define text widths \standard, \proceedings and \myletter.
%% \proceedings prints a single, narrow column near the edge of the page.
%% Use these before \begin{document} command.
%%
\def\standard{\oddsidemargin=0in
              \evensidemargin=0in
              \topmargin =-.5in
              \textheight=8.5in
              \textwidth=6.5in}
\def\proceedings{\oddsidemargin=-.5in
                 \evensidemargin=-.5in
                 \textwidth=4.56in
                 \parindent=0.3in
                 \topmargin=-1in
                 \textheight=10in
                 \pagestyle{empty}}
\def\myletter{\oddsidemargin=.3in
                 \evensidemargin=.3in
                 \baselineskip=16pt
                 \textwidth=5.5in
                 \pagestyle{empty}}
%%
%% Define command to pull in letterhead file.
%% This command is specific to VAX/VMS and Arbortext dvips program.
%% Insert your own path.
%%
\def\letterhead{\special{ps: plotfile [is.nelson.com]letterhead.tex 
local}}
%%
%%
%% LISTS:
%% Define \plainlist environment
%%
\newenvironment{plainlist}
{\begin{list}%
{}{\setlength{\leftmargin}{\rightmargin}\setlength{\labelwidth}{0in}}}%
{\end{list}}
%%
%% Define \hangref environment for hanging indentation
%%
\newenvironment{hangref}{\begin{list}{}{\setlength{\itemsep}{0pt}%
\setlength{\parsep}{0pt}\setlength{\leftmargin}{+\parindent}%
\setlength{\itemindent}{-\parindent}}}{\end{list}}
%%
%%
%%
%%
%% MATHEMATICS:
%%Special math symbols
%%
%% operators
\def\E{{\rm E}}
\def\Var{{\rm Var}}
\def\Cov{{\rm Cov}}
\def\Corr{{\rm Corr}}
\def\Bias{{\rm Bias}}
\def\MSE{{\rm MSE}}
\def\CP{{\rm CP}}
\def\trace{{\rm trace}}
\def\tr{{\rm tr}}
%%
%% bold face roman
\def\bA{{\bf A}}
\def\ba{{\bf a}}
\def\bB{{\bf B}}
\def\bb{{\bf b}}
\def\bC{{\bf C}}
\def\bc{{\bf c}}
\def\bD{{\bf D}}
\def\bd{{\bf d}}
\def\bE{{\bf E}}
\def\be{{\bf e}}
\def\bF{{\bf F}}
\def\boldf{{\bf f}}
\def\bG{{\bf G}}
\def\bg{{\bf g}}
\def\bH{{\bf H}}
\def\bh{{\bf h}}
\def\bi{{\bf i}}
\def\bI{{\bf I}}
\def\bJ{{\bf J}}
\def\bj{{\bf j}}
\def\bK{{\bf K}}
\def\bk{{\bf k}}
\def\bL{{\bf L}}
\def\bl{{\bf l}}
\def\bM{{\bf M}}
\def\bm{{\bf m}}
\def\bN{{\bf N}}
\def\bn{{\bf n}}
\def\bO{{\bf O}}
\def\bo{{\bf o}}
\def\bP{{\bf P}}
\def\bp{{\bf p}}
\def\bQ{{\bf Q}}
\def\bq{{\bf q}}
\def\bR{{\bf R}}
\def\br{{\bf r}}
\def\bS{{\bf S}}
\def\bs{{\bf s}}
\def\bT{{\bf T}}
\def\bt{{\bf t}}
\def\bU{{\bf U}}
\def\bu{{\bf u}}
\def\bV{{\bf V}}
\def\bv{{\bf v}}
\def\bW{{\bf W}}
\def\bw{{\bf w}}
\def\bX{{\bf X}}
\def\bx{{\bf x}}
\def\bY{{\bf Y}}
\def\by{{\bf y}}
\def\bZ{{\bf Z}}
\def\bz{{\bf z}}
%%
%% bold face Greek (incomplete)
\def\balpha{\mbox{\boldmath $\alpha$}}
\def\bbeta{\mbox{\boldmath $\beta$}}
\def\bepsilon{\mbox{\boldmath $\epsilon$}}
\def\bvarepsilon{\mbox{\boldmath $\varepsilon$}}
\def\bDelta{{\bf \Delta}}
\def\bdelta{\mbox{\boldmath $\delta$}}
\def\boldeta{\mbox{\boldmath $\eta$}}
\def\bGamma{{\bf \Gamma}}
\def\bgamma{\mbox{\boldmath $\gamma$}}
\def\bLambda{{\bf \Lambda}}
\def\blambda{\mbox{\boldmath $\lambda$}}
\def\bmu{\mbox{\boldmath $\mu$}}
\def\bOmega{{\bf \Omega}}
\def\bpi{\mbox{\boldmath $\pi$}}
\def\bphi{\mbox{\boldmath $\phi$}}
\def\bPsi{{\bf \Psi}}
\def\bpsi{\mbox{\boldmath $\psi$}}
\def\bSigma{{\bf \Sigma}}
\def\bsigma{\mbox{\boldmath $\sigma$}}
\def\bTheta{{\bf \Theta}}
\def\btheta{\mbox{\boldmath $\theta$}}
\def\bXi{{\bf \Xi}}
\def\bxi{\mbox{\boldmath $\xi$}}
%%
%% misc. Greek with hats
\def\betahat{\hat \beta}
\def\bbetahat{\hat{\mbox{\boldmath $\beta$}}}
\def\bdeltahat{\hat{\mbox{\boldmath $\delta$}}}
\def\etahat{\hat{\eta}}
\def\epsilonhat{\hat{\epsilon}}
\def\bepsilonhat{\hat{\mbox{\boldmath $\epsilon$}}}
\def\bgammahat{\hat{\mbox{\boldmath $\gamma$}}}
\def\bmuhat{\hat{\mbox{\boldmath $\mu$}}}
\def\thetahat{\hat \theta}
%%
%% caligraphy letters
\def\cA{{\cal A}}
\def\cB{{\cal B}}
\def\cC{{\cal C}}
\def\cD{{\cal D}}
\def\cE{{\cal E}}
\def\cI{{\cal I}}
\def\cM{{\cal M}}
\def\cR{{\cal R}}
\def\cS{{\cal S}}
\def\cT{{\cal T}}
\def\cY{{\cal Y}}
%%
%% tt letters
\def\tS{{\tt S}}
\def\tC{{\tt C}}
\def\tI{{\tt I}}
\def\tT{{\tt T}}
%%
%% vec notation
\def\vp{\vec{p}}
\def\bvP{\vec{{\bf P}}}
%%
%% bold face numbers
\def\b1{{\bf 1}}
\def\bzero{{\bf 0}}
%%
%% \blot gives a square at end of formulas and proofs
%% (thanks to Marc Posner)
\def\blot{\quad {$\vcenter{\vbox{\hrule height.4pt
             \hbox{\vrule width.4pt height.9ex \kern.9ex \vrule 
width.4pt}
             \hrule height.4pt}}$}}
%%
%% End of latexmacro

==> wscbib.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                            %
%     THESE COMMANDS ARE REQUIRED TO WORK WITH WSC.BST TO MAKE BIBLIO     %
%                                                                            %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\let\@internalcite\cite
%
\def\cite{\def\@citeseppen{-1000}%
    \def\@cite##1##2{(##1\if@tempswa , ##2\fi)}%
    \def\citeauthoryear##1##2##3{##1 ##3}\@internalcite}
\def\citeNP{\def\@citeseppen{-1000}%
    \def\@cite##1##2{##1\if@tempswa , ##2\fi}%
    \def\citeauthoryear##1##2##3{##1 ##3}\@internalcite}
\def\citeN{\def\@citeseppen{-1000}%
%  Pierre L'Ecuyer's fix for multiple cite bug
%  Added by Paul J Sanchez on 4 October 2001
%   \def\@cite##1##2{##1\if@tempswa , ##2)\else{)}\fi}%
%   \def\citeauthoryear##1##2##3{##1 (##3}\@citedata}
    \def\@cite##1##2{##1\if@tempswa, ##2)\else{}\fi}%
    \def\citeauthoryear##1##2##3{##1 (##3)}\@citedata}
\def\citeA{\def\@citeseppen{-1000}%
    \def\@cite##1##2{(##1\if@tempswa , ##2\fi)}%
    \def\citeauthoryear##1##2##3{##1}\@internalcite}
\def\citeANP{\def\@citeseppen{-1000}%
    \def\@cite##1##2{##1\if@tempswa , ##2\fi}%
    \def\citeauthoryear##1##2##3{##1}\@internalcite}
%
\def\shortcite{\def\@citeseppen{-1000}%
    \def\@cite##1##2{(##1\if@tempswa , ##2\fi)}%
    \def\citeauthoryear##1##2##3{##2 ##3}\@internalcite}
\def\shortciteNP{\def\@citeseppen{-1000}%
    \def\@cite##1##2{##1\if@tempswa , ##2\fi}%
    \def\citeauthoryear##1##2##3{##2 ##3}\@internalcite}
\def\shortciteN{\def\@citeseppen{-1000}%
%  Pierre L'Ecuyer's fix for multiple cite bug
%  Added by Paul J Sanchez on 2 September 2002
%  should have caught this last year...
%   \def\@cite##1##2{##1\if@tempswa , ##2)\else{)}\fi}%
%   \def\citeauthoryear##1##2##3{##2 (##3}\@citedata}
% Shane G. Henderson fix for extra right bracket at end of optional material June 8, 2005
%    \def\@cite##1##2{##1\if@tempswa, ##2)\else{}\fi}%
    \def\@cite##1##2{##1\if@tempswa, ##2\else{}\fi}%
    \def\citeauthoryear##1##2##3{##2 (##3)}\@citedata}
\def\shortciteA{\def\@citeseppen{-1000}%
    \def\@cite##1##2{(##1\if@tempswa , ##2\fi)}%
    \def\citeauthoryear##1##2##3{##2}\@internalcite}
\def\shortciteANP{\def\@citeseppen{-1000}%
    \def\@cite##1##2{##1\if@tempswa , ##2\fi}%
    \def\citeauthoryear##1##2##3{##2}\@internalcite}
%
\def\citeyear{\def\@citeseppen{-1000}%
    \def\@cite##1##2{(##1\if@tempswa , ##2\fi)}%
    \def\citeauthoryear##1##2##3{##3}\@citedata}
\def\citeyearNP{\def\@citeseppen{-1000}%
    \def\@cite##1##2{##1\if@tempswa , ##2\fi}%
    \def\citeauthoryear##1##2##3{##3}\@citedata}
%
% \@citedata and \@citedatax:
%
% Place commas in-between citations in the same \citeyear, \citeyearNP,
% \citeN, or \shortciteN command.
% Use something like \citeN{ref1,ref2,ref3} and \citeN{ref4} for a list.
%
\def\@citedata{%
    \@ifnextchar [{\@tempswatrue\@citedatax}%
                  {\@tempswafalse\@citedatax[]}%
}

\def\@citedatax[#1]#2{%
\if@filesw\immediate\write\@auxout{\string\citation{#2}}\fi%
  \def\@citea{}\@cite{\@for\@citeb:=#2\do%
    {\@citea\def\@citea{, }\@ifundefined% by Young
       {b@\@citeb}{{\bf ?}%
       \@warning{Citation `\@citeb' on page \thepage \space undefined}}%
{\csname b@\@citeb\endcsname}}}{#1}}%

% don't box citations, separate with ; and a space
% also, make the penalty between citations negative: a good place to break.
%
\def\@citex[#1]#2{%
\if@filesw\immediate\write\@auxout{\string\citation{#2}}\fi%
  \def\@citea{}\@cite{\@for\@citeb:=#2\do%
    {\@citea\def\@citea{; }\@ifundefined% by Young
       {b@\@citeb}{{\bf ?}%
       \@warning{Citation `\@citeb' on page \thepage \space undefined}}%
{\csname b@\@citeb\endcsname}}}{#1}}%

% (from apalike.sty)
% No labels in the bibliography.
%
\def\@biblabel#1{}
\makeatother

%\newlength{\bibhang}
%\setlength{\bibhang}{2em}

% Indent second and subsequent lines of bibliographic entries. Taken
% from openbib.sty: \newblock is set to {}.
% \renewcommand{\refname}{REFERENCES}

\newdimen\bibindent
\bibindent=0.0em
% SEC: was \def\thebibliography#1{\section*{\refname\@mkboth
% SEC: was   {\uppercase{\refname}}{\uppercase{\refname}}}\list
\def\thebibliography#1{\section*{\refname}\list
   {}{\settowidth\labelwidth{[#1]}
   \leftmargin\parindent
   \itemindent -\parindent
   \listparindent \itemindent
   \itemsep 0pt
   \parsep 0pt}
   \def\newblock{}
   \sloppy
   \sfcode`\.=1000\relax}



